MotionCraft: Crafting Whole-Body Motion with Plug-and-Play Multimodal Controls

Whole-body multimodal motion generation, controlled by text, speech, or music, has numerous applications including video generation and character animation. However, employing a unified model to achieve various generation tasks with different condition modalities presents two main challenges: motion distribution drifts across different tasks (e.g., co-speech gestures and text-driven daily actions) and the complex optimization of mixed conditions with varying granularities (e.g., text and audio). Additionally, inconsistent motion formats across different tasks and datasets hinder effective training toward multimodal motion generation. In this paper, we propose MotionCraft, a unified diffusion transformer that crafts whole-body motion with plug-and-play multimodal control. Our framework employs a coarse-to-fine training strategy, starting with the first stage of text-to-motion semantic pre-training, followed by the second stage of multimodal low-level control adaptation to handle conditions of varying granularities. To effectively learn and transfer motion knowledge across different distributions, we design MC-Attn for parallel modeling of static and dynamic human topology graphs. To overcome the motion format inconsistency of existing benchmarks, we introduce MC-Bench, the first available multimodal whole-body motion generation benchmark based on the unified SMPL-X format. Extensive experiments show that MotionCraft achieves state-of-the-art performance on various standard motion generation tasks.

==> tables/4-M2D-eval.tex <==
\begin{table}
    \centering
    % \vspace{-0.3cm}
    \resizebox{0.90\linewidth}{!}{
        \begin{tabular}{c|ccc}
            % \hline
            \toprule
            {Method} & {$FID_{H}$ $\downarrow$} & {$FID_{B}$ $\downarrow$} & {Div $\uparrow$} \\
            % \cline{2-3}
            % & Acc. $\uparrow$ & I2I. $\downarrow$ & & & \\ 
            \hline
            
            Edge & $93.430$ & $108.507$ & $13.471$ \\ 
            Finedance & $10.747$ & \cellcolor{red!15}$72.229$ & $13.813$ \\ 
            MCM & \cellcolor{yellow!15}$4.717$ & $78.577$ & $14.890$ \\ 
            \hline
            \OurMethod-Basic & \cellcolor{red!15}$3.858$ & \cellcolor{yellow!15}$76.248$ & \cellcolor{yellow!15}$16.667$ \\ 
            % \OurMethod-Mix & \cellcolor{yellow!15}$4.237$ & $185.930$ & \cellcolor{red!15}$21.278$ \\ 
            \OurMethod-Mix & 4.825 & 124.935 & \cellcolor{red!15}20.742 \\ 
            % \hline
            \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Results of music-to-dance in FineDance of \Benchmark.}
    We evaluate the $FID_{H}$, $FID_{B}$, and the diversity of \OurMethod~and SOTA baselines.
    $\colorbox{red!15}{\rm Indicate best results}, \colorbox{yellow!15}{\rm indicates second best results}$.}
    \label{tab:m2d_res_1}
    \vspace{-0.5cm}
\end{table}
